Block-STM: Scaling Blockchain Execution by Turning Ordering Curse to a Performance Blessing

Block-STM is a parallel execution engine for smart contracts, built around the principles of Software Transactional Memory. Transactions are grouped in blocks, and every execution of the block must yield the same deterministic outcome. Block-STM further enforces that the outcome is consistent with executing transactions according to a preset order, leveraging this order to dynamically detect dependencies and avoid conflicts during speculative transaction execution. At the core of Block-STM is a novel, low-overhead collaborative scheduler of execution and validation tasks. Block-STM is implemented on the main branch of the Diem Blockchain code-base and runs in production at Aptos. Our evaluation demonstrates that Block-STM is adaptive to workloads with different conflict rates and utilizes the inherent parallelism therein. Block-STM achieves up to $110k$ tps in the Diem benchmarks and up to $170k$ tps in the Aptos Benchmarks, which is a $20$x and $17$x improvement over the sequential baseline with $32$ threads, respectively. The throughput on a contended workload is up to $50k$ tps and $80k$ tps in Diem and Aptos benchmarks, respectively.

==> alg-main.tex <==
\begin{algorithm*}[h]
    \caption{Main}
    \label{alg:init}
    \small
    \begin{algorithmic}[1]
    
    \Procedure{\rust{main}}{\emph{block}}
        \State \rust{BLOCK} $\gets$ \emph{block}
    
        \For{$\emph{i} \in [0, \rust{NUM\_THREADS)}]$}
            \State \rust{thread.spawn(\emph{i})}
        \EndFor
        
        \State \textbf{upon threads join}
        \Indent
            \State \module{Storage}\rust{.persist(\module{MVMemory}.\emph{snapshot()})} \Comment{persist the final state into storage}
            \label{line:persist}
        \EndIndent
    \EndProcedure
    \alglinenoNew{counter}
    \alglinenoPush{counter}
    \end{algorithmic}
\end{algorithm*}


==> graphs.tex <==

\begin{figure}[t]
    \centering
    \pgfplotsset{footnotesize,height=4.5cm, width=\linewidth}
    \begin{tikzpicture}
    \begin{axis}[
        scaled y ticks=base 10:-3,
        legend columns=10,
        legend style={font=\footnotesize, at={(-0.1,1.35)},anchor=north west,legend columns=2},
        xlabel={Number of threads},
        ylabel= {Throughput},
        grid=major,
        xtick={4, 8, 16, 24, 32},
        ymin=0,
        ]
        \addplot [line width=0.25mm, color=red, mark=diamond] table [x=threads, y=litm10k,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, black, mark=square] [error bars/.cd, y explicit,y dir=both,] table [x=threads, y=seq,  col sep=comma] {plots/simple-batch-10k};
        \addlegendentry{BSTM, $10^3$ acc}
        \addlegendentry{BSTM, $10^4$ acc}
        \addlegendentry{LiTM, $10^3$ acc}
        \addlegendentry{LiTM, $10^4$ acc}
        \addlegendentry{Sequential}
        \addlegendentry{\textsc{Bohm}, $10^3$ acc}
        \addlegendentry{\textsc{Bohm}, $10^4$ acc}
    \end{axis}
    \end{tikzpicture}
    \label{fig:all-1k-sp2p}


 \label{fig:all-sp2p}
\end{figure}




\begin{figure}[t]
    \centering
    \pgfplotsset{footnotesize,height=4.5cm, width=\linewidth}
    \begin{tikzpicture}
    \begin{axis}[
        scaled y ticks=base 10:-3,
        legend columns=2,
        % legend pos=north west,
        % legend pos=outer north,
        legend style={font=\footnotesize, at={(0.0,1.7)},anchor=north west,legend columns=2},
        xlabel={Number of threads},
        ylabel= {Throughput},
        grid=major,
        xtick={4, 8, 16, 24, 32},
        % ytick={0,1.8,8.2,20.4},
        % ymax=25,
        ymin = 0,
        ]
        %
        \addplot [line width=0.25mm, color=magenta, mark=triangle] table [x=threads, y=bstm2,  col sep=comma] {plots/simple-batch-1k};
        %
        \addplot [line width=0.25mm, color=blue, mark=triangle] table [x=threads, y=bstm10,  col sep=comma] {plots/simple-batch-1k};
        %
        \addplot [line width=0.25mm, color=cyan, mark=triangle] table [x=threads, y=bstm100,  col sep=comma] {plots/simple-batch-1k};
        %
        \addplot [line width=0.25mm, color=yellow, mark=diamond] table [x=threads, y=bstm2,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, color=green, mark=diamond] table [x=threads, y=bstm10,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, color=red, mark=diamond] table [x=threads, y=bstm100,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, black, mark=square] [error bars/.cd, y explicit,y dir=both,] table [x=threads, y=seq,  col sep=comma] {plots/simple-batch-1k};
        %
        \addlegendentry{BSTM, 2 acc, $10^3$ bch}
        \addlegendentry{BSTM, 10 acc, $10^3$ bch}
        \addlegendentry{BSTM, 100 acc, $10^3$ bch}
        \addlegendentry{BSTM, 2 acc, $10^4$ bch}
        \addlegendentry{BSTM, 10 acc, $10^4$ bch}
        \addlegendentry{BSTM, 100 acc, $10^4$ bch}
        \addlegendentry{Sequential}
    \end{axis}
    \end{tikzpicture}
    \caption{Comparison of BSTM and sequential execution for batch size $10^3$ and $10^4$, account sizes 2, 10 and 100.}
    \label{fig:bstm-high-sp2p}
\end{figure}



\begin{figure}[t]
    \centering
    \pgfplotsset{footnotesize,height=4.5cm, width=\linewidth}
    \begin{tikzpicture}
    \begin{axis}[
        scaled y ticks=base 10:-3,
        legend columns=2,
        % legend pos=north west,
        % legend pos=outer north,
        legend style={font=\footnotesize, at={(0.0,1.7)},anchor=north west,legend columns=2},
        xlabel={Number of threads},
        ylabel= {Throughput},
        grid=major,
        xtick={4, 8, 16, 24, 32},
        % ytick={0,1.8,8.2,20.4},
        % ymax=25,
        ymin = 0,
        ]
        %
        \addplot [line width=0.25mm, color=magenta, mark=triangle] table [x=threads, y=bstm2,  col sep=comma] {plots/simple-batch-1k};
        %
        \addplot [line width=0.25mm, color=blue, mark=triangle] table [x=threads, y=bstm10,  col sep=comma] {plots/simple-batch-1k};
        %
        \addplot [line width=0.25mm, color=cyan, mark=triangle] table [x=threads, y=bstm100,  col sep=comma] {plots/simple-batch-1k};
        %
        \addplot [line width=0.25mm, color=yellow, mark=diamond] table [x=threads, y=bstm2,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, color=green, mark=diamond] table [x=threads, y=bstm10,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, color=red, mark=diamond] table [x=threads, y=bstm100,  col sep=comma] {plots/simple-batch-10k};
        %
        \addplot [line width=0.25mm, black, mark=square] [error bars/.cd, y explicit,y dir=both,] table [x=threads, y=seq,  col sep=comma] {plots/simple-batch-1k};
        %
        \addlegendentry{BSTM, 2 acc, $10^3$ bch}
        \addlegendentry{BSTM, 10 acc, $10^3$ bch}
        \addlegendentry{BSTM, 100 acc, $10^3$ bch}
        \addlegendentry{BSTM, 2 acc, $10^4$ bch}
        \addlegendentry{BSTM, 10 acc, $10^4$ bch}
        \addlegendentry{BSTM, 100 acc, $10^4$ bch}
        \addlegendentry{Sequential}
    \end{axis}
    \end{tikzpicture}
    \caption{Comparison of BSTM and sequential execution for batch size $10^3$ and $10^4$, account sizes 2, 10 and 100.}
    \label{fig:bstm-high-sp2p}
\end{figure}




==> schduling.tex <==
\section{Validation Scheduling}

The \STMBFT scheduler dispatches validation tasks greedily and optimistically in parallel. When validation fails is causes re-execution. This has a ripple effect, requiring all tasks higher than the execution index to re-validate, potentially effectuating more re-executions. Executions and validations are carried concurrently. In order to coordinate validation dispatching, we maintain a monotonically increasing logical clock, \rust{TS}. For each transaction \rust{tid} in the block, the algorithm records:

\begin{itemize}
    \item \rust{E\_TS(tid)}, a timestamp \rust{TS} at the latest execution's completion time, initially zero.
    \item \rust{V\_TS(tid)}, a timestamp \rust{TS} at the latest validation dispatch time, initially zero.
\end{itemize}

When a transaction \rust{tid}'s execution completes, it atomically records the current logical time \rust{TS} and increments it. When a transaction is dispatched for validation, it records the current logical time \rust{TS}.

Scheduling validation task $vid$ becomes a simple matter of querying whether all executions up to $vid$ have completed, and whether one of them has completed at a time later than $vid$'s latest validation time. 

%In order to support these queries efficiently, maximal and minimal \rust{E\_TS} accumulators are maintained in a tree, as depicted below in Figure~\ref{fig:sched}. 
%and increments it? I don't think it is needed
%Accumulators are updated at execution completion as follows:

\begin{description}
\item[Upon \rust{tid}'s completion:] \mbox{} 

    \begin{itemize}
        \item \rust{E\_TS(tid) := fetch\_and\_increments(TS)}.
 %       \item For $i=1 .. \log(n)$, update max/min \rust{E\_TS} at transaction $kid = k_i * n/(n^i)$, where $k_i$ is the smallest index s.t.\ $k_i * n/(2^i) \geq tid$.

    \end{itemize}
\item[Upon start of \rust{tid}'s validation:]  \mbox{} 

    \begin{itemize}
        \item \rust{V\_TS(tid) := fetch(TS)}
    \end{itemize}
\end{description} 

\noindent
Validation dispatching picks a transaction \rust{tid} satisfying the following:

\begin{enumerate}
    \item The latest execution of \rust{tid} has completed.
    \item The maximal \rust{E\_TS} of transactions preceding \rust{tid} is higher than \rust{V\_TS(tid)}.
    \item The minimal \rust{E\_TS} of transactions preceding \rust{tid} is greater than zero.
\end{enumerate}

The scenario in Figure~\ref{fig:sched} shows a system after 8 transactions have been dispatched for execution; transactions 1-4 have completed their execution at timestamps 1-4, respectively; validations of 1-4 have been dispatched at timestamp 4; transaction 5 has completed at timestamp 5;  transaction 3 has been aborted and its re-execution completed at timestamp 6. Validations of transactions 3,4 and 5 are pending next.   

\begin{figure}[h]
\centering{
\includegraphics[width=0.75\textwidth]{images/schedule.png}
}
\caption{An example schedule with timestamps recorded.}
\label{fig:sched}
\end{figure}


